Machine learning approach for early detection of autism by combining questionnaire and home video screening

Existing screening tools for early detection of autism are expensive, cumbersome, time-intensive, and sometimes fall short in predictive value. In this work, we apply Machine Learning (ML) to gold standard clinical data obtained across thousands of children at risk for autism spectrum disorders to create a low-cost, quick, and easy to apply autism screening tool that performs as well or better than most widely used standardized instruments. This new tool combines two screening methods into a single assessment, one based on short, structured parent-report questionnaires and the other on tagging key behaviors from short, semi-structured home videos of children. To overcome the scarcity, sparsity, and imbalance of training data, we apply creative feature selection, feature engineering, and novel feature encoding techniques. We allow for inconclusive determination where appropriate in order to boost screening accuracy when conclusive. We demonstrate a significant accuracy improvement over standard screening tools in a clinical study sample of 162 children.

==> images/ADOS2_average_recall.tex <==
\begin{tabular}{cccccccc}
\toprule
max features & criterion & max depth &  n trees & Scalar, all features & Scalar, restricted features & Encoded, restricted features &    Proportional loss \\
\midrule
        log2 &      gini &         4 &       50 &  $0.6705 \pm 0.0011$ &          $0.6764 \pm 0.001$ &          $0.6692 \pm 0.0011$ &  $0.5704 \pm 0.0011$ \\
        log2 &   entropy &         4 &      200 &  $0.6657 \pm 0.0009$ &         $0.6749 \pm 0.0012$ &           $0.672 \pm 0.0009$ &  $0.5698 \pm 0.0017$ \\
        log2 &      gini &         4 &      200 &  $0.6645 \pm 0.0009$ &         $0.6761 \pm 0.0013$ &          $0.6781 \pm 0.0009$ &  $0.5691 \pm 0.0016$ \\
        log2 &   entropy &         4 &      150 &  $0.6683 \pm 0.0008$ &         $0.6788 \pm 0.0012$ &           $0.6723 \pm 0.001$ &  $0.5684 \pm 0.0011$ \\
        log2 &      gini &         4 &      150 &  $0.6661 \pm 0.0008$ &         $0.6811 \pm 0.0014$ &           $0.675 \pm 0.0007$ &  $0.5677 \pm 0.0009$ \\
        log2 &   entropy &         4 &       50 &  $0.6628 \pm 0.0008$ &          $0.678 \pm 0.0013$ &           $0.6724 \pm 0.001$ &  $0.5664 \pm 0.0009$ \\
        log2 &      gini &         5 &      100 &  $0.6675 \pm 0.0007$ &         $0.6762 \pm 0.0008$ &          $0.6757 \pm 0.0008$ &  $0.5654 \pm 0.0016$ \\
        log2 &      gini &         4 &      100 &  $0.6675 \pm 0.0007$ &         $0.6754 \pm 0.0008$ &            $0.676 \pm 0.001$ &  $0.5653 \pm 0.0012$ \\
        log2 &   entropy &         4 &      100 &  $0.6631 \pm 0.0009$ &         $0.6749 \pm 0.0013$ &           $0.6759 \pm 0.001$ &  $0.5649 \pm 0.0009$ \\
        None &   entropy &         4 &      100 &  $0.6696 \pm 0.0012$ &         $0.6715 \pm 0.0017$ &          $0.6584 \pm 0.0014$ &  $0.5647 \pm 0.0018$ \\
        log2 &      gini &         5 &      150 &  $0.6711 \pm 0.0006$ &         $0.6807 \pm 0.0006$ &          $0.6795 \pm 0.0008$ &   $0.5635 \pm 0.001$ \\
        log2 &      gini &         5 &      200 &  $0.6707 \pm 0.0007$ &         $0.6844 \pm 0.0011$ &          $0.6761 \pm 0.0008$ &    $0.563 \pm 0.001$ \\
        None &      gini &         4 &      100 &  $0.6619 \pm 0.0014$ &          $0.669 \pm 0.0013$ &          $0.6609 \pm 0.0017$ &  $0.5627 \pm 0.0019$ \\
        log2 &   entropy &         5 &      200 &  $0.6689 \pm 0.0011$ &         $0.6814 \pm 0.0009$ &          $0.6773 \pm 0.0007$ &  $0.5626 \pm 0.0011$ \\
        None &      gini &         4 &       50 &   $0.6614 \pm 0.002$ &         $0.6696 \pm 0.0009$ &          $0.6615 \pm 0.0014$ &   $0.562 \pm 0.0014$ \\
        log2 &   entropy &         5 &      150 &  $0.6663 \pm 0.0008$ &         $0.6749 \pm 0.0005$ &          $0.6734 \pm 0.0009$ &  $0.5619 \pm 0.0013$ \\
        log2 &   entropy &         6 &      200 &  $0.6656 \pm 0.0006$ &         $0.6762 \pm 0.0013$ &          $0.6783 \pm 0.0008$ &   $0.5614 \pm 0.001$ \\
        None &   entropy &         4 &      200 &  $0.6617 \pm 0.0013$ &         $0.6713 \pm 0.0012$ &          $0.6629 \pm 0.0016$ &  $0.5613 \pm 0.0013$ \\
        None &      gini &         4 &      150 &  $0.6642 \pm 0.0008$ &         $0.6722 \pm 0.0011$ &          $0.6544 \pm 0.0011$ &  $0.5611 \pm 0.0018$ \\
        log2 &   entropy &         5 &      100 &   $0.667 \pm 0.0005$ &         $0.6787 \pm 0.0009$ &            $0.679 \pm 0.001$ &   $0.5607 \pm 0.001$ \\
\bottomrule
\end{tabular}


==> tables/ADOS1_average_recall.tex <==
\begin{tabular}{cccccccc}
\toprule
max features & criterion & max depth &  n trees & Scalar, all features & Scalar, restricted features & Encoded, restricted features &    Proportional loss \\
\midrule
        log2 &   entropy &         4 &      200 &  $0.6565 \pm 0.0005$ &         $0.6599 \pm 0.0007$ &           $0.655 \pm 0.0005$ &  $0.5651 \pm 0.0007$ \\
        None &      gini &         4 &       50 &  $0.6563 \pm 0.0008$ &         $0.6532 \pm 0.0006$ &          $0.6458 \pm 0.0006$ &  $0.5648 \pm 0.0009$ \\
        None &      gini &         4 &      100 &  $0.6581 \pm 0.0007$ &         $0.6567 \pm 0.0007$ &           $0.645 \pm 0.0009$ &  $0.5635 \pm 0.0007$ \\
        log2 &   entropy &         4 &      150 &  $0.6576 \pm 0.0005$ &         $0.6525 \pm 0.0006$ &          $0.6567 \pm 0.0005$ &  $0.5628 \pm 0.0009$ \\
        log2 &   entropy &         4 &       50 &  $0.6561 \pm 0.0005$ &         $0.6574 \pm 0.0005$ &          $0.6555 \pm 0.0007$ &  $0.5624 \pm 0.0009$ \\
        None &   entropy &         4 &       50 &  $0.6553 \pm 0.0007$ &         $0.6563 \pm 0.0011$ &          $0.6443 \pm 0.0006$ &  $0.5623 \pm 0.0011$ \\
        None &      gini &         4 &      200 &   $0.653 \pm 0.0008$ &          $0.657 \pm 0.0007$ &          $0.6468 \pm 0.0007$ &  $0.5622 \pm 0.0007$ \\
        None &   entropy &         4 &      150 &   $0.652 \pm 0.0008$ &         $0.6549 \pm 0.0008$ &          $0.6476 \pm 0.0007$ &  $0.5621 \pm 0.0008$ \\
        log2 &      gini &         5 &       50 &   $0.654 \pm 0.0006$ &         $0.6567 \pm 0.0007$ &          $0.6487 \pm 0.0005$ &  $0.5621 \pm 0.0008$ \\
        None &   entropy &         4 &      100 &  $0.6542 \pm 0.0006$ &         $0.6544 \pm 0.0008$ &          $0.6465 \pm 0.0007$ &   $0.5619 \pm 0.001$ \\
        log2 &   entropy &         4 &      100 &  $0.6572 \pm 0.0006$ &         $0.6582 \pm 0.0007$ &          $0.6559 \pm 0.0006$ &  $0.5619 \pm 0.0008$ \\
        log2 &      gini &         4 &      150 &  $0.6612 \pm 0.0007$ &         $0.6581 \pm 0.0007$ &          $0.6529 \pm 0.0006$ &  $0.5614 \pm 0.0006$ \\
        None &      gini &         4 &      150 &   $0.651 \pm 0.0008$ &         $0.6541 \pm 0.0009$ &          $0.6474 \pm 0.0006$ &  $0.5612 \pm 0.0011$ \\
        log2 &      gini &         4 &      100 &  $0.6565 \pm 0.0004$ &         $0.6594 \pm 0.0006$ &          $0.6571 \pm 0.0005$ &  $0.5612 \pm 0.0008$ \\
        None &   entropy &         4 &      200 &  $0.6549 \pm 0.0007$ &         $0.6586 \pm 0.0007$ &          $0.6462 \pm 0.0009$ &  $0.5612 \pm 0.0005$ \\
        log2 &      gini &         4 &       50 &  $0.6545 \pm 0.0006$ &         $0.6573 \pm 0.0008$ &          $0.6511 \pm 0.0005$ &  $0.5605 \pm 0.0008$ \\
        log2 &   entropy &         5 &      100 &  $0.6523 \pm 0.0007$ &         $0.6569 \pm 0.0007$ &          $0.6481 \pm 0.0007$ &  $0.5605 \pm 0.0004$ \\
        log2 &      gini &         5 &      100 &  $0.6567 \pm 0.0006$ &         $0.6567 \pm 0.0005$ &          $0.6484 \pm 0.0007$ &  $0.5596 \pm 0.0008$ \\
        log2 &      gini &         5 &      150 &  $0.6561 \pm 0.0006$ &          $0.652 \pm 0.0004$ &           $0.648 \pm 0.0005$ &  $0.5586 \pm 0.0007$ \\
        log2 &   entropy &         5 &      150 &  $0.6526 \pm 0.0004$ &         $0.6564 \pm 0.0008$ &          $0.6505 \pm 0.0007$ &  $0.5584 \pm 0.0006$ \\
\bottomrule
\end{tabular}


==> tables/ADOS2_average_recall.tex <==
\begin{tabular}{cccccccc}
\toprule
max features & criterion & max depth &  n trees & Scalar, all features & Scalar, restricted features & Encoded, restricted features &    Proportional loss \\
\midrule
        log2 &      gini &         4 &       50 &  $0.6705 \pm 0.0011$ &          $0.6764 \pm 0.001$ &          $0.6692 \pm 0.0011$ &  $0.5704 \pm 0.0011$ \\
        log2 &   entropy &         4 &      200 &  $0.6657 \pm 0.0009$ &         $0.6749 \pm 0.0012$ &           $0.672 \pm 0.0009$ &  $0.5698 \pm 0.0017$ \\
        log2 &      gini &         4 &      200 &  $0.6645 \pm 0.0009$ &         $0.6761 \pm 0.0013$ &          $0.6781 \pm 0.0009$ &  $0.5691 \pm 0.0016$ \\
        log2 &   entropy &         4 &      150 &  $0.6683 \pm 0.0008$ &         $0.6788 \pm 0.0012$ &           $0.6723 \pm 0.001$ &  $0.5684 \pm 0.0011$ \\
        log2 &      gini &         4 &      150 &  $0.6661 \pm 0.0008$ &         $0.6811 \pm 0.0014$ &           $0.675 \pm 0.0007$ &  $0.5677 \pm 0.0009$ \\
        log2 &   entropy &         4 &       50 &  $0.6628 \pm 0.0008$ &          $0.678 \pm 0.0013$ &           $0.6724 \pm 0.001$ &  $0.5664 \pm 0.0009$ \\
        log2 &      gini &         5 &      100 &  $0.6675 \pm 0.0007$ &         $0.6762 \pm 0.0008$ &          $0.6757 \pm 0.0008$ &  $0.5654 \pm 0.0016$ \\
        log2 &      gini &         4 &      100 &  $0.6675 \pm 0.0007$ &         $0.6754 \pm 0.0008$ &            $0.676 \pm 0.001$ &  $0.5653 \pm 0.0012$ \\
        log2 &   entropy &         4 &      100 &  $0.6631 \pm 0.0009$ &         $0.6749 \pm 0.0013$ &           $0.6759 \pm 0.001$ &  $0.5649 \pm 0.0009$ \\
        None &   entropy &         4 &      100 &  $0.6696 \pm 0.0012$ &         $0.6715 \pm 0.0017$ &          $0.6584 \pm 0.0014$ &  $0.5647 \pm 0.0018$ \\
        log2 &      gini &         5 &      150 &  $0.6711 \pm 0.0006$ &         $0.6807 \pm 0.0006$ &          $0.6795 \pm 0.0008$ &   $0.5635 \pm 0.001$ \\
        log2 &      gini &         5 &      200 &  $0.6707 \pm 0.0007$ &         $0.6844 \pm 0.0011$ &          $0.6761 \pm 0.0008$ &    $0.563 \pm 0.001$ \\
        None &      gini &         4 &      100 &  $0.6619 \pm 0.0014$ &          $0.669 \pm 0.0013$ &          $0.6609 \pm 0.0017$ &  $0.5627 \pm 0.0019$ \\
        \textbf{log2} &   \textbf{entropy} &         \textbf{5} &      \textbf{200} &  $0.6689 \pm 0.0011$ &         $0.6814 \pm 0.0009$ &          $0.6773 \pm 0.0007$ &  $0.5626 \pm 0.0011$ \\
        None &      gini &         4 &       50 &   $0.6614 \pm 0.002$ &         $0.6696 \pm 0.0009$ &          $0.6615 \pm 0.0014$ &   $0.562 \pm 0.0014$ \\
        log2 &   entropy &         5 &      150 &  $0.6663 \pm 0.0008$ &         $0.6749 \pm 0.0005$ &          $0.6734 \pm 0.0009$ &  $0.5619 \pm 0.0013$ \\
        log2 &   entropy &         6 &      200 &  $0.6656 \pm 0.0006$ &         $0.6762 \pm 0.0013$ &          $0.6783 \pm 0.0008$ &   $0.5614 \pm 0.001$ \\
        None &   entropy &         4 &      200 &  $0.6617 \pm 0.0013$ &         $0.6713 \pm 0.0012$ &          $0.6629 \pm 0.0016$ &  $0.5613 \pm 0.0013$ \\
        None &      gini &         4 &      150 &  $0.6642 \pm 0.0008$ &         $0.6722 \pm 0.0011$ &          $0.6544 \pm 0.0011$ &  $0.5611 \pm 0.0018$ \\
        log2 &   entropy &         5 &      100 &   $0.667 \pm 0.0005$ &         $0.6787 \pm 0.0009$ &            $0.679 \pm 0.001$ &   $0.5607 \pm 0.001$ \\
\bottomrule
\end{tabular}


==> tables/clinical_optimization_results_questionnaire_combined.tex <==
\begin{tabular}{p{3.5cm}|p{1cm}p{1cm}p{1cm}|p{1cm}p{1cm}p{1cm}|p{1cm}p{1cm}p{1cm}}
\hline
 & \multicolumn{3}{|c|}{AUC} & \multicolumn{3}{c|}{Average precision} & \multicolumn{3}{c}{Specificity} \\
scenario &  All&  $< 4$&  $\geq 4$&  All&  $< 4$&  $\geq 4$&  All&  $< 4$&  $\geq 4$\\

\hline
age silo                 &   0.4626 &     0.3876 &        0.5127 &                          0.4734 &                            0.3818 &                               0.5345 &          0.1762 &            0.0833 &               0.2381 \\
with encoding            &   0.6719 &     0.6859 &        0.6626 &                          0.6288 &                            0.6481 &                               0.6159 &          0.4119 &            0.4583 &               0.3810 \\
with feature engineering &   0.7003 &     0.7264 &        0.6829 &                          0.6875 &                            0.7287 &                               0.6601 &          0.5357 &            0.6250 &               0.4762 \\
With 25\% inconclusive allowance &   0.7003 &     0.7264 &        0.6829 &                          0.7276 &                            0.7575 &                               0.7076 &          0.5857 &            0.7143 &               0.5000 \\
\hline
\end{tabular}


==> tables/clinical_optimized_performance.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
               latex\_scenario &  triton.3- &  triton.4+ &   ADOS1 &   ADOS2 &  train triton.3- &  train triton.4+ &  train ADOS1 &  train ADOS2 \\
                              &            &            &         &         &                  &                  &              &              \\
\midrule
         Scalar, all features &        NaN &        NaN &     NaN &     NaN &           0.8714 &           0.9003 &       0.6612 &       0.6711 \\
  Scalar, restricted features &     0.5910 &     0.5633 &  0.7652 &  0.5650 &           0.8663 &           0.8723 &       0.6621 &       0.6844 \\
 Encoded, restricted features &     0.6195 &     0.5740 &  0.6926 &  0.5934 &           0.8651 &           0.8818 &       0.6571 &       0.6811 \\
            Proportional loss &        NaN &        NaN &  0.6360 &  0.5702 &              NaN &              NaN &       0.5651 &       0.5704 \\
                   Exact prod &     0.5987 &     0.5633 &  0.7368 &  0.6227 &           0.8586 &           0.8818 &       0.5584 &       0.5626 \\
\bottomrule
\end{tabular}


==> tables/clinical_optimized_performance_AUC.tex <==
\begin{tabular}{lrrr}
\toprule
{} &   young &     old &  all ages \\
AUC                      &         &         &           \\
\midrule
Age binned               &  0.3876 &  0.5127 &    0.4626 \\
With encoding            &  0.6859 &  0.6626 &    0.6719 \\
With feature engineering &  0.7105 &  0.6545 &    0.6769 \\
\bottomrule
\end{tabular}


==> tables/clinical_optimized_performance_autism_recall.tex <==
\begin{tabular}{lrrr}
\toprule
{} &   young &     old &  all ages \\
Autism Recall            &         &         &           \\
\midrule
Age binned               &  1.0000 &  1.0000 &    1.0000 \\
With encoding            &  0.9605 &  0.8723 &    0.9076 \\
With feature engineering &  0.9474 &  0.8723 &    0.9024 \\
\bottomrule
\end{tabular}


==> tables/clinical_optimized_performance_average_precision_reallife.tex <==
\begin{tabular}{lrrr}
\toprule
{} &   young &     old &  all ages \\
Average Precision [Reallife] &         &         &           \\
\midrule
Age binned                   &     NaN &  0.7625 &       NaN \\
With encoding                &  0.6945 &  0.6204 &    0.6501 \\
With feature engineering     &  0.6921 &  0.6449 &    0.6638 \\
\bottomrule
\end{tabular}


==> tables/clinical_optimized_performance_average_recall.tex <==
\begin{tabular}{lrrr}
\toprule
{} &   young &     old &  all ages \\
Average Recall           &         &         &           \\
\midrule
Age binned               &  0.5000 &  0.5476 &    0.5286 \\
With encoding            &  0.5844 &  0.5790 &    0.5812 \\
With feature engineering &  0.5987 &  0.6028 &    0.6012 \\
\bottomrule
\end{tabular}


==> tables/clinical_optimized_performance_not_recall.tex <==
\begin{tabular}{lrrr}
\toprule
{} &   young &     old &  all ages \\
Not Recall               &         &         &           \\
\midrule
Age binned               &  0.0000 &  0.0952 &    0.0571 \\
With encoding            &  0.2083 &  0.2857 &    0.2548 \\
With feature engineering &  0.2500 &  0.3333 &    0.3000 \\
\bottomrule
\end{tabular}


==> tables/optimized_performance.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
               latex\_scenario &  triton.3- &  triton.4+ &     ADOS1 &     ADOS2 &  train triton.3- &  train triton.4+ &  train ADOS1 &  train ADOS2 \\
\midrule
         Scalar, all features &        NaN &        NaN &       NaN &       NaN &         0.871413 &         0.900271 &     0.661227 &     0.671063 \\
  Scalar, restricted features &   0.591009 &   0.563323 &  0.765224 &  0.564956 &         0.866335 &         0.872341 &     0.662106 &     0.684396 \\
 Encoded, restricted features &   0.619518 &   0.573961 &  0.692575 &  0.593424 &         0.865079 &         0.881810 &     0.657091 &     0.681144 \\
            Proportional loss &        NaN &        NaN &  0.635951 &  0.570168 &              NaN &              NaN &     0.565074 &     0.570442 \\
                   Used for clinical study &   0.598684 &   0.563323 &  0.736779 &  0.622694 &              0.8586 &              0.8818 &          0.5584 &          0.5626 \\
\bottomrule
\end{tabular}


==> tables/optimized_performance_AUC.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  triton.3- &  triton.4+ &  train triton.3- &  train triton.4+ \\
AUC                                      &            &            &                  &                  \\
\midrule
triton features, age binned, no encoding &     0.3876 &     0.5127 &           0.9108 &           0.9606 \\
triton features, with encoding           &     0.6859 &     0.6626 &           0.9234 &           0.9622 \\
triton features, encoding, engineering   &     0.7105 &     0.6515 &           0.9213 &           0.9647 \\
\bottomrule
\end{tabular}


==> tables/optimized_performance_autism_recall.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  triton.3- &  triton.4+ &  train triton.3- &  train triton.4+ \\
Autism Recall                            &            &            &                  &                  \\
\midrule
triton features, age binned, no encoding &     1.0000 &     1.0000 &           0.9335 &           0.9662 \\
triton features, with encoding           &     0.9605 &     0.8723 &           0.9243 &           0.9726 \\
triton features, encoding, engineering   &     0.9474 &     0.8723 &           0.9381 &           0.9618 \\
\bottomrule
\end{tabular}


==> tables/optimized_performance_average_precision_reallife.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  triton.3- &  triton.4+ &  train triton.3- &  train triton.4+ \\
Average Precision [Reallife]             &            &            &                  &                  \\
\midrule
triton features, age binned, no encoding &        NaN &     0.7625 &           0.8564 &           0.8724 \\
triton features, with encoding           &     0.6945 &     0.6204 &           0.8523 &           0.8827 \\
triton features, encoding, engineering   &     0.6921 &     0.6449 &           0.8568 &           0.8931 \\
\bottomrule
\end{tabular}


==> tables/optimized_performance_average_recall.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  triton.3- &  triton.4+ &  train triton.3- &  train triton.4+ \\
Average Recall                           &            &            &                  &                  \\
\midrule
triton features, age binned, no encoding &     0.5000 &     0.5476 &           0.8451 &           0.8532 \\
triton features, with encoding           &     0.5844 &     0.5790 &           0.8429 &           0.8648 \\
triton features, encoding, engineering   &     0.5987 &     0.6028 &           0.8441 &           0.8833 \\
\bottomrule
\end{tabular}


==> tables/optimized_performance_average_recall_old.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  triton.3- &  triton.4+ &   ADOS1 &   ADOS2 &  train triton.3- &  train triton.4+ &  train ADOS1 &  train ADOS2 \\
Average Recall               &            &            &         &         &                  &                  &              &              \\
\midrule
Scalar, all features         &        NaN &        NaN &     NaN &     NaN &         0.871400 &         0.900300 &     0.661200 &     0.671100 \\
Scalar, restricted features  &     0.5910 &     0.5633 &  0.7652 &  0.5650 &         0.866300 &         0.872300 &     0.662100 &     0.684400 \\
Encoded, restricted features &     0.6195 &     0.5740 &  0.6926 &  0.5934 &         0.865100 &         0.881800 &     0.657100 &     0.681100 \\
Proportional loss            &        NaN &        NaN &  0.6360 &  0.5702 &              NaN &              NaN &     0.565100 &     0.570400 \\
Exact prod                   &     0.5987 &     0.5633 &  0.7368 &  0.6227 &         0.821256 &         0.793884 &     0.563756 &     0.558172 \\
\bottomrule
\end{tabular}


==> tables/optimized_performance_not_recall.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &  triton.3- &  triton.4+ &  train triton.3- &  train triton.4+ \\
Not Recall                               &            &            &                  &                  \\
\midrule
triton features, age binned, no encoding &     0.0000 &     0.0952 &           0.7567 &           0.7402 \\
triton features, with encoding           &     0.2083 &     0.2857 &           0.7615 &           0.7571 \\
triton features, encoding, engineering   &     0.2500 &     0.3333 &           0.7501 &           0.8048 \\
\bottomrule
\end{tabular}


==> tables/training_data_demographic_details.tex <==
\begin{tabular}{lcc}
\toprule
{} &  Autism &  Not autism \\
Age in years &         &             \\
\midrule
2            &     134 &          53 \\
3            &     280 &         154 \\
4            &     662 &          59 \\
5            &     625 &          75 \\
6            &     598 &          46 \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_AUC.tex <==
\begin{tabular}{cccc}
\toprule
                     AUC &                young &                  old &             combined \\
                         &                      &                      &                      \\
\midrule
             Base method &  $0.9542 \pm 0.0127$ &  $0.9542 \pm 0.0127$ &  $0.9542 \pm 0.0092$ \\
 Tally feature selection &  $0.9574 \pm 0.0002$ &  $0.9574 \pm 0.0002$ &  $0.9574 \pm 0.0001$ \\
              Age binned &  $0.9467 \pm 0.0006$ &  $0.9682 \pm 0.0002$ &  $0.9596 \pm 0.0003$ \\
           With encoding &   $0.951 \pm 0.0003$ &  $0.9697 \pm 0.0003$ &  $0.9623 \pm 0.0002$ \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_AUC_no_official_requirement.tex <==
\begin{tabular}{cccc}
\toprule
                      AUC &            young &              old &          combined \\
                          &                  &                  &                   \\
\midrule
              Base method &  0.9415 to 0.967 &  0.9415 to 0.967 &  0.9451 to 0.9634 \\
  Tally feature selection &           0.9574 &           0.9574 &            0.9574 \\
               Age binned &           0.9467 &           0.9682 &            0.9596 \\
            With encoding &            0.951 &           0.9697 &            0.9623 \\
 With feature engineering &           0.9771 &            0.966 &            0.9704 \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_autism_precision__Reallife__no_official_requirement.tex <==
\begin{tabular}{cccc}
\toprule
autism precision [Reallife] &             young &               old &          combined \\
                            &                   &                   &                   \\
\midrule
                Base method &  0.7552 to 0.8013 &  0.7552 to 0.8013 &  0.7616 to 0.7948 \\
    Tally feature selection &            0.7794 &            0.7794 &            0.7794 \\
                 Age binned &            0.8316 &            0.8206 &             0.825 \\
              With encoding &            0.8412 &            0.7971 &            0.8148 \\
   With feature engineering &            0.8996 &            0.7739 &            0.8242 \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_autism_recall.tex <==
\begin{tabular}{cccc}
\toprule
           autism recall &                young &                  old &             combined \\
                         &                      &                      &                      \\
\midrule
             Base method &  $0.9591 \pm 0.0059$ &  $0.9591 \pm 0.0059$ &  $0.9591 \pm 0.0042$ \\
 Tally feature selection &  $0.9639 \pm 0.0003$ &  $0.9639 \pm 0.0003$ &  $0.9639 \pm 0.0002$ \\
              Age binned &   $0.896 \pm 0.0009$ &  $0.9784 \pm 0.0002$ &  $0.9454 \pm 0.0004$ \\
           With encoding &  $0.9047 \pm 0.0012$ &  $0.9894 \pm 0.0001$ &  $0.9555 \pm 0.0005$ \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_autism_recall_no_official_requirement.tex <==
\begin{tabular}{cccc}
\toprule
            autism recall &            young &              old &          combined \\
                          &                  &                  &                   \\
\midrule
              Base method &  0.9533 to 0.965 &  0.9533 to 0.965 &  0.9549 to 0.9633 \\
  Tally feature selection &           0.9639 &           0.9639 &            0.9639 \\
               Age binned &            0.896 &           0.9784 &            0.9454 \\
            With encoding &           0.9047 &           0.9894 &            0.9555 \\
 With feature engineering &           0.9846 &           0.9884 &            0.9869 \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_average_precision__Reallife__no_official_requirement.tex <==
\begin{tabular}{cccc}
\toprule
average precision [Reallife] &             young &               old &          combined \\
                             &                   &                   &                   \\
\midrule
                 Base method &  0.8497 to 0.8758 &  0.8497 to 0.8758 &  0.8533 to 0.8722 \\
     Tally feature selection &             0.866 &             0.866 &             0.866 \\
                  Age binned &            0.8594 &            0.8969 &            0.8819 \\
               With encoding &            0.8692 &            0.8916 &            0.8826 \\
    With feature engineering &            0.9413 &            0.8789 &            0.9039 \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_average_recall.tex <==
\begin{tabular}{cccc}
\toprule
          average recall &                young &                  old &             combined \\
                         &                      &                      &                      \\
\midrule
             Base method &  $0.8428 \pm 0.0181$ &  $0.8428 \pm 0.0181$ &   $0.8428 \pm 0.013$ \\
 Tally feature selection &   $0.8454 \pm 0.001$ &   $0.8454 \pm 0.001$ &  $0.8454 \pm 0.0007$ \\
              Age binned &   $0.8571 \pm 0.001$ &  $0.8822 \pm 0.0007$ &  $0.8721 \pm 0.0006$ \\
           With encoding &   $0.8668 \pm 0.001$ &  $0.8687 \pm 0.0006$ &   $0.868 \pm 0.0005$ \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_average_recall_no_official_requirement.tex <==
\begin{tabular}{cccc}
\toprule
           average recall &             young &               old &          combined \\
                          &                   &                   &                   \\
\midrule
              Base method &  0.8247 to 0.8608 &  0.8247 to 0.8608 &  0.8297 to 0.8558 \\
  Tally feature selection &            0.8454 &            0.8454 &            0.8454 \\
               Age binned &            0.8571 &            0.8822 &            0.8721 \\
            With encoding &            0.8668 &            0.8687 &             0.868 \\
 With feature engineering &            0.9373 &            0.8498 &            0.8848 \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_not_precision__Reallife__no_official_requirement.tex <==
\begin{tabular}{cccc}
\toprule
 not precision [Reallife] &             young &               old &          combined \\
                          &                   &                   &                   \\
\midrule
              Base method &  0.9402 to 0.9543 &  0.9402 to 0.9543 &  0.9422 to 0.9524 \\
  Tally feature selection &            0.9527 &            0.9527 &            0.9527 \\
               Age binned &            0.8873 &            0.9733 &            0.9389 \\
            With encoding &            0.8972 &             0.986 &            0.9505 \\
 With feature engineering &            0.9831 &             0.984 &            0.9836 \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_not_recall.tex <==
\begin{tabular}{cccc}
\toprule
              not recall &                young &                  old &             combined \\
                         &                      &                      &                      \\
\midrule
             Base method &  $0.7264 \pm 0.0371$ &  $0.7264 \pm 0.0371$ &  $0.7264 \pm 0.0268$ \\
 Tally feature selection &   $0.7268 \pm 0.002$ &   $0.7268 \pm 0.002$ &  $0.7268 \pm 0.0014$ \\
              Age binned &  $0.8182 \pm 0.0018$ &   $0.786 \pm 0.0015$ &  $0.7989 \pm 0.0011$ \\
           With encoding &  $0.8289 \pm 0.0015$ &  $0.7481 \pm 0.0011$ &  $0.7804 \pm 0.0009$ \\
\bottomrule
\end{tabular}


==> tables/training_optimization_results_questionnaire_not_recall_no_official_requirement.tex <==
\begin{tabular}{cccc}
\toprule
               not recall &             young &               old &          combined \\
                          &                   &                   &                   \\
\midrule
              Base method &  0.6893 to 0.7635 &  0.6893 to 0.7635 &  0.6996 to 0.7532 \\
  Tally feature selection &            0.7268 &            0.7268 &            0.7268 \\
               Age binned &            0.8182 &             0.786 &            0.7989 \\
            With encoding &            0.8289 &            0.7481 &            0.7804 \\
 With feature engineering &              0.89 &            0.7111 &            0.7827 \\
\bottomrule
\end{tabular}


==> tables/triton.3-_average_recall.tex <==
\begin{tabular}{ccccccc}
\toprule
max features & criterion & max depth &  n trees & Scalar, all features & Scalar, restricted features & Encoded, restricted features \\
\midrule
        log2 &   entropy &         8 &      150 &  $0.8626 \pm 0.0006$ &         $0.8611 \pm 0.0005$ &          $0.8651 \pm 0.0007$ \\
        log2 &   entropy &         6 &      200 &  $0.8714 \pm 0.0006$ &         $0.8646 \pm 0.0006$ &          $0.8645 \pm 0.0008$ \\
        log2 &      gini &         5 &      200 &    $0.87 \pm 0.0007$ &         $0.8614 \pm 0.0004$ &          $0.8643 \pm 0.0008$ \\
        log2 &      gini &         8 &      200 &  $0.8656 \pm 0.0008$ &          $0.862 \pm 0.0005$ &          $0.8627 \pm 0.0006$ \\
        None &   entropy &         6 &       50 &   $0.869 \pm 0.0007$ &         $0.8654 \pm 0.0009$ &           $0.862 \pm 0.0007$ \\
        None &   entropy &         5 &       50 &  $0.8524 \pm 0.0009$ &         $0.8658 \pm 0.0007$ &          $0.8617 \pm 0.0006$ \\
        log2 &      gini &         6 &      150 &  $0.8625 \pm 0.0006$ &         $0.8648 \pm 0.0006$ &          $0.8616 \pm 0.0007$ \\
        None &      gini &         5 &      100 &  $0.8655 \pm 0.0009$ &         $0.8568 \pm 0.0007$ &          $0.8612 \pm 0.0007$ \\
        log2 &   entropy &         8 &      100 &  $0.8651 \pm 0.0005$ &         $0.8645 \pm 0.0006$ &          $0.8605 \pm 0.0011$ \\
        log2 &      gini &         8 &      150 &  $0.8642 \pm 0.0007$ &         $0.8606 \pm 0.0008$ &          $0.8605 \pm 0.0007$ \\
        log2 &      gini &         4 &      100 &  $0.8635 \pm 0.0005$ &         $0.8629 \pm 0.0006$ &          $0.8593 \pm 0.0007$ \\
        log2 &   entropy &         6 &      100 &  $0.8681 \pm 0.0007$ &         $0.8655 \pm 0.0006$ &          $0.8592 \pm 0.0009$ \\
        log2 &   entropy &         5 &      100 &   $0.866 \pm 0.0005$ &         $0.8603 \pm 0.0007$ &          $0.8592 \pm 0.0008$ \\
        log2 &      gini &         6 &      200 &  $0.8679 \pm 0.0007$ &         $0.8604 \pm 0.0007$ &          $0.8589 \pm 0.0008$ \\
        None &   entropy &         5 &      200 &  $0.8621 \pm 0.0016$ &         $0.8641 \pm 0.0007$ &          $0.8588 \pm 0.0006$ \\
        log2 &      gini &         5 &      150 &  $0.8668 \pm 0.0006$ &         $0.8581 \pm 0.0005$ &          $0.8587 \pm 0.0007$ \\
        \textbf{log2} &   \textbf{entropy} &         \textbf{5} &      \textbf{150} &  $0.8697 \pm 0.0007$ &         $0.8611 \pm 0.0005$ &          $0.8586 \pm 0.0007$ \\
        log2 &   entropy &         5 &       50 &  $0.8674 \pm 0.0006$ &         $0.8596 \pm 0.0005$ &          $0.8586 \pm 0.0007$ \\
        log2 &      gini &         8 &      100 &  $0.8639 \pm 0.0008$ &          $0.8612 \pm 0.001$ &          $0.8585 \pm 0.0006$ \\
        None &   entropy &         6 &      150 &  $0.8601 \pm 0.0009$ &         $0.8629 \pm 0.0011$ &          $0.8585 \pm 0.0006$ \\
\bottomrule
\end{tabular}


==> tables/triton.4+_average_recall.tex <==
\begin{tabular}{ccccccc}
\toprule
max features & criterion & max depth &  n trees & Scalar, all features & Scalar, restricted features & Encoded, restricted features \\
\midrule
        None &   entropy &         4 &      100 &  $0.8699 \pm 0.0008$ &         $0.8515 \pm 0.0008$ &          $0.8982 \pm 0.0007$ \\
        None &   entropy &         4 &      150 &  $0.8695 \pm 0.0008$ &         $0.8537 \pm 0.0008$ &           $0.8943 \pm 0.001$ \\
        None &   entropy &         4 &      200 &  $0.8687 \pm 0.0007$ &         $0.8512 \pm 0.0008$ &          $0.8934 \pm 0.0008$ \\
        None &   entropy &         4 &       50 &  $0.8688 \pm 0.0011$ &         $0.8493 \pm 0.0007$ &          $0.8902 \pm 0.0008$ \\
        None &      gini &         4 &      150 &  $0.8794 \pm 0.0008$ &         $0.8549 \pm 0.0009$ &          $0.8897 \pm 0.0007$ \\
        None &   entropy &         5 &      100 &  $0.8523 \pm 0.0013$ &         $0.8431 \pm 0.0007$ &          $0.8874 \pm 0.0009$ \\
        None &      gini &         4 &      200 &   $0.8755 \pm 0.001$ &          $0.852 \pm 0.0005$ &           $0.8856 \pm 0.001$ \\
        None &      gini &         4 &       50 &  $0.8753 \pm 0.0011$ &         $0.8563 \pm 0.0008$ &           $0.885 \pm 0.0012$ \\
        None &   entropy &         5 &      150 &  $0.8565 \pm 0.0005$ &          $0.8447 \pm 0.001$ &          $0.8833 \pm 0.0012$ \\
        None &      gini &         4 &      100 &  $0.8795 \pm 0.0012$ &         $0.8541 \pm 0.0012$ &           $0.883 \pm 0.0011$ \\
        \textbf{log2} &   \textbf{entropy} &         \textbf{5} &      \textbf{150} &  $0.8837 \pm 0.0009$ &         $0.8643 \pm 0.0006$ &          $0.8818 \pm 0.0007$ \\
        log2 &      gini &         5 &       50 &  $0.8792 \pm 0.0009$ &         $0.8622 \pm 0.0011$ &          $0.8812 \pm 0.0005$ \\
        None &   entropy &         5 &       50 &   $0.854 \pm 0.0007$ &         $0.8432 \pm 0.0007$ &           $0.8798 \pm 0.001$ \\
        log2 &      gini &         5 &      200 &  $0.8927 \pm 0.0009$ &         $0.8665 \pm 0.0004$ &          $0.8797 \pm 0.0006$ \\
        log2 &   entropy &         5 &      100 &  $0.8859 \pm 0.0008$ &         $0.8633 \pm 0.0007$ &          $0.8794 \pm 0.0006$ \\
        log2 &      gini &         5 &      100 &   $0.8873 \pm 0.001$ &         $0.8646 \pm 0.0006$ &          $0.8789 \pm 0.0005$ \\
        None &   entropy &         5 &      200 &  $0.8552 \pm 0.0007$ &         $0.8445 \pm 0.0007$ &          $0.8787 \pm 0.0007$ \\
        log2 &   entropy &         5 &      200 &  $0.8899 \pm 0.0006$ &         $0.8629 \pm 0.0008$ &          $0.8785 \pm 0.0006$ \\
        log2 &   entropy &         5 &       50 &    $0.883 \pm 0.001$ &           $0.864 \pm 0.001$ &          $0.8784 \pm 0.0006$ \\
        log2 &      gini &         5 &      150 &  $0.8865 \pm 0.0009$ &         $0.8649 \pm 0.0008$ &           $0.878 \pm 0.0006$ \\
\bottomrule
\end{tabular}


==> tables_old/ADOS1_average_recall.tex <==
\begin{tabular}{llllrrrrr}
\toprule
{} & max\_features & criterion & max\_depth &  n\_trees &  Scalar, all features average recall &  Scalar, restricted features average recall &  Encoded, restricted features average recall &  Proportional loss average recall \\
\midrule
0  &         None &   entropy &        10 &       50 &                             0.599455 &                                    0.598055 &                                     0.610017 &                          0.523791 \\
1  &         None &   entropy &        10 &      100 &                             0.597443 &                                    0.596492 &                                     0.604177 &                          0.521482 \\
2  &         None &   entropy &        10 &      150 &                             0.599016 &                                    0.592132 &                                     0.606382 &                          0.526877 \\
3  &         None &   entropy &        10 &      200 &                             0.602566 &                                    0.597379 &                                     0.604343 &                          0.525748 \\
4  &         None &   entropy &         4 &       50 &                             0.655283 &                                    0.656302 &                                     0.644253 &                          0.562291 \\
5  &         None &   entropy &         4 &      100 &                             0.654166 &                                    0.654365 &                                     0.646544 &                          0.561889 \\
6  &         None &   entropy &         4 &      150 &                             0.651965 &                                    0.654871 &                                     0.647596 &                          0.562130 \\
7  &         None &   entropy &         4 &      200 &                             0.654935 &                                    0.658570 &                                     0.646185 &                          0.561241 \\
8  &         None &   entropy &         5 &       50 &                             0.650709 &                                    0.652121 &                                     0.641298 &                          0.550167 \\
9  &         None &   entropy &         5 &      100 &                             0.649293 &                                    0.651317 &                                     0.641297 &                          0.553942 \\
10 &         None &   entropy &         5 &      150 &                             0.657350 &                                    0.654666 &                                     0.645269 &                          0.553623 \\
11 &         None &   entropy &         5 &      200 &                             0.651177 &                                    0.650962 &                                     0.641823 &                          0.555297 \\
12 &         None &   entropy &         6 &       50 &                             0.645751 &                                    0.648298 &                                     0.641446 &                          0.541889 \\
13 &         None &   entropy &         6 &      100 &                             0.644561 &                                    0.648719 &                                     0.639518 &                          0.538004 \\
14 &         None &   entropy &         6 &      150 &                             0.644148 &                                    0.643989 &                                     0.632078 &                          0.540895 \\
15 &         None &   entropy &         6 &      200 &                             0.645634 &                                    0.647749 &                                     0.639616 &                          0.540345 \\
16 &         None &   entropy &         8 &       50 &                             0.623629 &                                    0.628840 &                                     0.617090 &                          0.527412 \\
17 &         None &   entropy &         8 &      100 &                             0.620489 &                                    0.623021 &                                     0.613041 &                          0.527089 \\
18 &         None &   entropy &         8 &      150 &                             0.624366 &                                    0.624643 &                                     0.615415 &                          0.522634 \\
19 &         None &   entropy &         8 &      200 &                             0.628340 &                                    0.622509 &                                     0.613148 &                          0.530658 \\
20 &         None &   entropy &      None &       50 &                             0.557935 &                                    0.563275 &                                     0.606152 &                          0.523334 \\
21 &         None &   entropy &      None &      100 &                             0.555732 &                                    0.562499 &                                     0.608713 &                          0.522525 \\
22 &         None &   entropy &      None &      150 &                             0.559173 &                                    0.566129 &                                     0.606708 &                          0.521264 \\
23 &         None &   entropy &      None &      200 &                             0.558732 &                                    0.567162 &                                     0.605665 &                          0.521918 \\
24 &         None &      gini &        10 &       50 &                             0.599548 &                                    0.590561 &                                     0.604960 &                          0.515481 \\
25 &         None &      gini &        10 &      100 &                             0.599456 &                                    0.591159 &                                     0.606147 &                          0.525383 \\
26 &         None &      gini &        10 &      150 &                             0.596265 &                                    0.591778 &                                     0.602956 &                          0.519160 \\
27 &         None &      gini &        10 &      200 &                             0.596145 &                                    0.588946 &                                     0.607618 &                          0.517454 \\
28 &         None &      gini &         4 &       50 &                             0.656293 &                                    0.653170 &                                     0.645785 &                          0.564756 \\
29 &         None &      gini &         4 &      100 &                             0.658096 &                                    0.656667 &                                     0.645016 &                          0.563541 \\
30 &         None &      gini &         4 &      150 &                             0.651007 &                                    0.654071 &                                     0.647412 &                          0.561209 \\
31 &         None &      gini &         4 &      200 &                             0.652958 &                                    0.656953 &                                     0.646821 &                          0.562208 \\
32 &         None &      gini &         5 &       50 &                             0.651242 &                                    0.655001 &                                     0.645704 &                          0.551183 \\
33 &         None &      gini &         5 &      100 &                             0.651920 &                                    0.650639 &                                     0.642097 &                          0.553664 \\
34 &         None &      gini &         5 &      150 &                             0.653233 &                                    0.652559 &                                     0.646198 &                          0.552800 \\
35 &         None &      gini &         5 &      200 &                             0.653771 &                                    0.656394 &                                     0.646297 &                          0.552744 \\
36 &         None &      gini &         6 &       50 &                             0.648448 &                                    0.643573 &                                     0.633076 &                          0.544069 \\
37 &         None &      gini &         6 &      100 &                             0.648194 &                                    0.648599 &                                     0.637036 &                          0.539777 \\
38 &         None &      gini &         6 &      150 &                             0.652522 &                                    0.649071 &                                     0.636807 &                          0.535816 \\
39 &         None &      gini &         6 &      200 &                             0.645563 &                                    0.648626 &                                     0.634076 &                          0.539090 \\
40 &         None &      gini &         8 &       50 &                             0.619577 &                                    0.618545 &                                     0.614366 &                          0.527648 \\
41 &         None &      gini &         8 &      100 &                             0.625010 &                                    0.619757 &                                     0.612129 &                          0.524646 \\
42 &         None &      gini &         8 &      150 &                             0.625923 &                                    0.618175 &                                     0.613185 &                          0.525926 \\
43 &         None &      gini &         8 &      200 &                             0.624039 &                                    0.617933 &                                     0.613483 &                          0.526740 \\
44 &         None &      gini &      None &       50 &                             0.552667 &                                    0.555521 &                                     0.608115 &                          0.526786 \\
45 &         None &      gini &      None &      100 &                             0.553440 &                                    0.558851 &                                     0.598257 &                          0.520495 \\
46 &         None &      gini &      None &      150 &                             0.558157 &                                    0.561352 &                                     0.605196 &                          0.521416 \\
47 &         None &      gini &      None &      200 &                             0.557843 &                                    0.554367 &                                     0.603658 &                          0.522157 \\
48 &         log2 &   entropy &        10 &       50 &                             0.605032 &                                    0.598447 &                                     0.599661 &                          0.520902 \\
49 &         log2 &   entropy &        10 &      100 &                             0.607764 &                                    0.601475 &                                     0.602950 &                          0.520814 \\
50 &         log2 &   entropy &        10 &      150 &                             0.605626 &                                    0.599047 &                                     0.605928 &                          0.522506 \\
51 &         log2 &   entropy &        10 &      200 &                             0.605688 &                                    0.599246 &                                     0.601984 &                          0.520345 \\
52 &         log2 &   entropy &         4 &       50 &                             0.656146 &                                    0.657367 &                                     0.655524 &                          0.562408 \\
53 &         log2 &   entropy &         4 &      100 &                             0.657182 &                                    0.658222 &                                     0.655947 &                          0.561923 \\
54 &         log2 &   entropy &         4 &      150 &                             0.657632 &                                    0.652513 &                                     0.656666 &                          0.562811 \\
55 &         log2 &   entropy &         4 &      200 &                             0.656497 &                                    0.659921 &                                     0.654996 &                          0.565074 \\
56 &         log2 &   entropy &         5 &       50 &                             0.653235 &                                    0.658866 &                                     0.648142 &                          0.557097 \\
57 &         log2 &   entropy &         5 &      100 &                             0.652309 &                                    0.656895 &                                     0.648077 &                          0.560472 \\
58 &         log2 &   entropy &         5 &      150 &                             0.652593 &                                    0.656449 &                                     0.650515 &                          0.558435 \\
59 &         log2 &   entropy &         5 &      200 &                             0.654231 &                                    0.657219 &                                     0.650588 &                          0.558050 \\
60 &         log2 &   entropy &         6 &       50 &                             0.649883 &                                    0.646124 &                                     0.643971 &                          0.550959 \\
61 &         log2 &   entropy &         6 &      100 &                             0.649223 &                                    0.650159 &                                     0.646181 &                          0.549337 \\
62 &         log2 &   entropy &         6 &      150 &                             0.653188 &                                    0.649993 &                                     0.642436 &                          0.550939 \\
63 &         log2 &   entropy &         6 &      200 &                             0.647597 &                                    0.648423 &                                     0.639357 &                          0.552290 \\
64 &         log2 &   entropy &         8 &       50 &                             0.632365 &                                    0.626469 &                                     0.619096 &                          0.530547 \\
65 &         log2 &   entropy &         8 &      100 &                             0.632793 &                                    0.626794 &                                     0.616747 &                          0.526285 \\
66 &         log2 &   entropy &         8 &      150 &                             0.636516 &                                    0.625468 &                                     0.616181 &                          0.531441 \\
67 &         log2 &   entropy &         8 &      200 &                             0.634766 &                                    0.630033 &                                     0.617847 &                          0.528219 \\
68 &         log2 &   entropy &      None &       50 &                             0.550715 &                                    0.561433 &                                     0.603976 &                          0.522505 \\
69 &         log2 &   entropy &      None &      100 &                             0.551681 &                                    0.563274 &                                     0.605190 &                          0.522068 \\
70 &         log2 &   entropy &      None &      150 &                             0.549145 &                                    0.560213 &                                     0.607329 &                          0.523902 \\
71 &         log2 &   entropy &      None &      200 &                             0.550477 &                                    0.563954 &                                     0.601905 &                          0.523304 \\
72 &         log2 &      gini &        10 &       50 &                             0.601660 &                                    0.598288 &                                     0.606550 &                          0.523310 \\
73 &         log2 &      gini &        10 &      100 &                             0.598805 &                                    0.600395 &                                     0.603205 &                          0.524630 \\
74 &         log2 &      gini &        10 &      150 &                             0.602449 &                                    0.596530 &                                     0.606974 &                          0.518699 \\
75 &         log2 &      gini &        10 &      200 &                             0.600953 &                                    0.598641 &                                     0.609237 &                          0.518465 \\
76 &         log2 &      gini &         4 &       50 &                             0.654490 &                                    0.657328 &                                     0.651127 &                          0.560515 \\
77 &         log2 &      gini &         4 &      100 &                             0.656465 &                                    0.659403 &                                     0.657091 &                          0.561170 \\
78 &         log2 &      gini &         4 &      150 &                             0.661227 &                                    0.658114 &                                     0.652937 &                          0.561429 \\
79 &         log2 &      gini &         4 &      200 &                             0.659234 &                                    0.662106 &                                     0.651685 &                          0.558330 \\
80 &         log2 &      gini &         5 &       50 &                             0.654035 &                                    0.656707 &                                     0.648660 &                          0.562075 \\
81 &         log2 &      gini &         5 &      100 &                             0.656680 &                                    0.656675 &                                     0.648381 &                          0.559640 \\
82 &         log2 &      gini &         5 &      150 &                             0.656060 &                                    0.651961 &                                     0.647998 &                          0.558581 \\
83 &         log2 &      gini &         5 &      200 &                             0.653194 &                                    0.658260 &                                     0.646756 &                          0.555850 \\
84 &         log2 &      gini &         6 &       50 &                             0.646779 &                                    0.652534 &                                     0.645662 &                          0.553181 \\
85 &         log2 &      gini &         6 &      100 &                             0.649074 &                                    0.651436 &                                     0.645567 &                          0.550865 \\
86 &         log2 &      gini &         6 &      150 &                             0.650513 &                                    0.649204 &                                     0.642684 &                          0.548635 \\
87 &         log2 &      gini &         6 &      200 &                             0.650317 &                                    0.649406 &                                     0.642010 &                          0.554638 \\
88 &         log2 &      gini &         8 &       50 &                             0.633523 &                                    0.622920 &                                     0.618768 &                          0.524734 \\
89 &         log2 &      gini &         8 &      100 &                             0.631306 &                                    0.627953 &                                     0.617272 &                          0.527972 \\
90 &         log2 &      gini &         8 &      150 &                             0.634225 &                                    0.625806 &                                     0.619094 &                          0.527056 \\
91 &         log2 &      gini &         8 &      200 &                             0.633186 &                                    0.624951 &                                     0.620142 &                          0.532636 \\
92 &         log2 &      gini &      None &       50 &                             0.546978 &                                    0.558735 &                                     0.606203 &                          0.526635 \\
93 &         log2 &      gini &      None &      100 &                             0.547463 &                                    0.556451 &                                     0.604773 &                          0.522755 \\
94 &         log2 &      gini &      None &      150 &                             0.550406 &                                    0.561128 &                                     0.601505 &                          0.525272 \\
95 &         log2 &      gini &      None &      200 &                             0.549255 &                                    0.560568 &                                     0.605557 &                          0.521288 \\
\bottomrule
\end{tabular}


==> tables_old/ADOS2_average_recall.tex <==
\begin{tabular}{llllrrrrr}
\toprule
{} & max\_features & criterion & max\_depth &  n\_trees &  Scalar, all features average recall &  Scalar, restricted features average recall &  Encoded, restricted features average recall &  Proportional loss average recall \\
\midrule
0  &         None &   entropy &        10 &       50 &                             0.617276 &                                    0.645970 &                                     0.658495 &                          0.538504 \\
1  &         None &   entropy &        10 &      100 &                             0.613274 &                                    0.639276 &                                     0.662879 &                          0.545770 \\
2  &         None &   entropy &        10 &      150 &                             0.618169 &                                    0.645970 &                                     0.658258 &                          0.537585 \\
3  &         None &   entropy &        10 &      200 &                             0.619606 &                                    0.640833 &                                     0.663255 &                          0.538646 \\
4  &         None &   entropy &         4 &       50 &                             0.660056 &                                    0.668154 &                                     0.661011 &                          0.558240 \\
5  &         None &   entropy &         4 &      100 &                             0.669552 &                                    0.671535 &                                     0.658418 &                          0.564654 \\
6  &         None &   entropy &         4 &      150 &                             0.662467 &                                    0.668586 &                                     0.661922 &                          0.555691 \\
7  &         None &   entropy &         4 &      200 &                             0.661660 &                                    0.671299 &                                     0.662879 &                          0.561291 \\
8  &         None &   entropy &         5 &       50 &                             0.665698 &                                    0.676392 &                                     0.666896 &                          0.553491 \\
9  &         None &   entropy &         5 &      100 &                             0.662711 &                                    0.676631 &                                     0.670634 &                          0.556173 \\
10 &         None &   entropy &         5 &      150 &                             0.659733 &                                    0.673365 &                                     0.674658 &                          0.557686 \\
11 &         None &   entropy &         5 &      200 &                             0.663838 &                                    0.680066 &                                     0.673117 &                          0.559014 \\
12 &         None &   entropy &         6 &       50 &                             0.660290 &                                    0.673167 &                                     0.668960 &                          0.545334 \\
13 &         None &   entropy &         6 &      100 &                             0.655703 &                                    0.674463 &                                     0.670448 &                          0.545574 \\
14 &         None &   entropy &         6 &      150 &                             0.661835 &                                    0.676947 &                                     0.681563 &                          0.545565 \\
15 &         None &   entropy &         6 &      200 &                             0.661234 &                                    0.674901 &                                     0.674792 &                          0.546730 \\
16 &         None &   entropy &         8 &       50 &                             0.639370 &                                    0.662888 &                                     0.670548 &                          0.537535 \\
17 &         None &   entropy &         8 &      100 &                             0.637547 &                                    0.658318 &                                     0.668711 &                          0.538314 \\
18 &         None &   entropy &         8 &      150 &                             0.639420 &                                    0.664986 &                                     0.669401 &                          0.534076 \\
19 &         None &   entropy &         8 &      200 &                             0.640145 &                                    0.663351 &                                     0.669535 &                          0.536930 \\
20 &         None &   entropy &      None &       50 &                             0.590255 &                                    0.611021 &                                     0.661503 &                          0.533334 \\
21 &         None &   entropy &      None &      100 &                             0.587354 &                                    0.614730 &                                     0.660873 &                          0.540784 \\
22 &         None &   entropy &      None &      150 &                             0.594407 &                                    0.613299 &                                     0.658669 &                          0.537664 \\
23 &         None &   entropy &      None &      200 &                             0.590633 &                                    0.615035 &                                     0.658609 &                          0.542671 \\
24 &         None &      gini &        10 &       50 &                             0.619176 &                                    0.633981 &                                     0.663580 &                          0.535795 \\
25 &         None &      gini &        10 &      100 &                             0.611188 &                                    0.633520 &                                     0.660258 &                          0.537166 \\
26 &         None &      gini &        10 &      150 &                             0.617342 &                                    0.634844 &                                     0.659408 &                          0.537447 \\
27 &         None &      gini &        10 &      200 &                             0.616956 &                                    0.635322 &                                     0.658673 &                          0.537538 \\
28 &         None &      gini &         4 &       50 &                             0.661436 &                                    0.669598 &                                     0.661547 &                          0.561977 \\
29 &         None &      gini &         4 &      100 &                             0.661876 &                                    0.668959 &                                     0.660855 &                          0.562667 \\
30 &         None &      gini &         4 &      150 &                             0.664220 &                                    0.672158 &                                     0.654367 &                          0.561057 \\
31 &         None &      gini &         4 &      200 &                             0.661226 &                                    0.671169 &                                     0.662448 &                          0.556676 \\
32 &         None &      gini &         5 &       50 &                             0.661482 &                                    0.674486 &                                     0.671807 &                          0.556248 \\
33 &         None &      gini &         5 &      100 &                             0.658647 &                                    0.676318 &                                     0.674644 &                          0.554128 \\
34 &         None &      gini &         5 &      150 &                             0.663438 &                                    0.676795 &                                     0.674710 &                          0.555812 \\
35 &         None &      gini &         5 &      200 &                             0.662677 &                                    0.675962 &                                     0.674770 &                          0.558415 \\
36 &         None &      gini &         6 &       50 &                             0.655409 &                                    0.672018 &                                     0.673409 &                          0.544733 \\
37 &         None &      gini &         6 &      100 &                             0.660007 &                                    0.672259 &                                     0.671883 &                          0.549723 \\
38 &         None &      gini &         6 &      150 &                             0.655337 &                                    0.678897 &                                     0.676097 &                          0.548750 \\
39 &         None &      gini &         6 &      200 &                             0.652999 &                                    0.673312 &                                     0.672248 &                          0.548636 \\
40 &         None &      gini &         8 &       50 &                             0.629477 &                                    0.655151 &                                     0.671271 &                          0.541640 \\
41 &         None &      gini &         8 &      100 &                             0.635144 &                                    0.657879 &                                     0.666190 &                          0.540494 \\
42 &         None &      gini &         8 &      150 &                             0.639016 &                                    0.663861 &                                     0.672829 &                          0.542011 \\
43 &         None &      gini &         8 &      200 &                             0.635447 &                                    0.657277 &                                     0.668554 &                          0.540392 \\
44 &         None &      gini &      None &       50 &                             0.583615 &                                    0.603552 &                                     0.660502 &                          0.539824 \\
45 &         None &      gini &      None &      100 &                             0.585288 &                                    0.608072 &                                     0.662743 &                          0.539596 \\
46 &         None &      gini &      None &      150 &                             0.592517 &                                    0.606498 &                                     0.666434 &                          0.546009 \\
47 &         None &      gini &      None &      200 &                             0.583202 &                                    0.604729 &                                     0.664432 &                          0.542107 \\
48 &         log2 &   entropy &        10 &       50 &                             0.636948 &                                    0.654615 &                                     0.665846 &                          0.534954 \\
49 &         log2 &   entropy &        10 &      100 &                             0.632893 &                                    0.648983 &                                     0.667343 &                          0.531860 \\
50 &         log2 &   entropy &        10 &      150 &                             0.633667 &                                    0.650417 &                                     0.657396 &                          0.532705 \\
51 &         log2 &   entropy &        10 &      200 &                             0.639369 &                                    0.652955 &                                     0.660829 &                          0.535826 \\
52 &         log2 &   entropy &         4 &       50 &                             0.662843 &                                    0.677967 &                                     0.672420 &                          0.566448 \\
53 &         log2 &   entropy &         4 &      100 &                             0.663099 &                                    0.674914 &                                     0.675869 &                          0.564931 \\
54 &         log2 &   entropy &         4 &      150 &                             0.668318 &                                    0.678796 &                                     0.672318 &                          0.568364 \\
55 &         log2 &   entropy &         4 &      200 &                             0.665667 &                                    0.674882 &                                     0.671967 &                          0.569769 \\
56 &         log2 &   entropy &         5 &       50 &                             0.666935 &                                    0.676660 &                                     0.678464 &                          0.559810 \\
57 &         log2 &   entropy &         5 &      100 &                             0.667025 &                                    0.678716 &                                     0.678958 &                          0.560745 \\
58 &         log2 &   entropy &         5 &      150 &                             0.666270 &                                    0.674921 &                                     0.673363 &                          0.561936 \\
59 &         log2 &   entropy &         5 &      200 &                             0.668937 &                                    0.681353 &                                     0.677327 &                          0.562606 \\
60 &         log2 &   entropy &         6 &       50 &                             0.662959 &                                    0.676172 &                                     0.679419 &                          0.556513 \\
61 &         log2 &   entropy &         6 &      100 &                             0.663856 &                                    0.677271 &                                     0.672062 &                          0.560635 \\
62 &         log2 &   entropy &         6 &      150 &                             0.667969 &                                    0.677339 &                                     0.679649 &                          0.556128 \\
63 &         log2 &   entropy &         6 &      200 &                             0.665602 &                                    0.676216 &                                     0.678324 &                          0.561430 \\
64 &         log2 &   entropy &         8 &       50 &                             0.646160 &                                    0.664157 &                                     0.674268 &                          0.540401 \\
65 &         log2 &   entropy &         8 &      100 &                             0.653215 &                                    0.669468 &                                     0.676660 &                          0.539989 \\
66 &         log2 &   entropy &         8 &      150 &                             0.653764 &                                    0.665435 &                                     0.674136 &                          0.546336 \\
67 &         log2 &   entropy &         8 &      200 &                             0.655838 &                                    0.667034 &                                     0.670238 &                          0.539997 \\
68 &         log2 &   entropy &      None &       50 &                             0.589056 &                                    0.618460 &                                     0.660963 &                          0.534443 \\
69 &         log2 &   entropy &      None &      100 &                             0.585028 &                                    0.612240 &                                     0.665527 &                          0.536666 \\
70 &         log2 &   entropy &      None &      150 &                             0.594057 &                                    0.621245 &                                     0.664324 &                          0.543114 \\
71 &         log2 &   entropy &      None &      200 &                             0.588880 &                                    0.619185 &                                     0.664547 &                          0.534709 \\
72 &         log2 &      gini &        10 &       50 &                             0.624853 &                                    0.649742 &                                     0.663505 &                          0.537005 \\
73 &         log2 &      gini &        10 &      100 &                             0.628527 &                                    0.644901 &                                     0.668642 &                          0.533505 \\
74 &         log2 &      gini &        10 &      150 &                             0.631688 &                                    0.648291 &                                     0.664522 &                          0.536556 \\
75 &         log2 &      gini &        10 &      200 &                             0.627682 &                                    0.652587 &                                     0.663888 &                          0.541928 \\
76 &         log2 &      gini &         4 &       50 &                             0.670468 &                                    0.676358 &                                     0.669209 &                          0.570442 \\
77 &         log2 &      gini &         4 &      100 &                             0.667485 &                                    0.675415 &                                     0.676037 &                          0.565299 \\
78 &         log2 &      gini &         4 &      150 &                             0.666084 &                                    0.681056 &                                     0.674982 &                          0.567721 \\
79 &         log2 &      gini &         4 &      200 &                             0.664536 &                                    0.676069 &                                     0.678099 &                          0.569078 \\
80 &         log2 &      gini &         5 &       50 &                             0.665367 &                                    0.680978 &                                     0.677863 &                          0.560582 \\
81 &         log2 &      gini &         5 &      100 &                             0.667494 &                                    0.676192 &                                     0.675713 &                          0.565411 \\
82 &         log2 &      gini &         5 &      150 &                             0.671063 &                                    0.680714 &                                     0.679513 &                          0.563479 \\
83 &         log2 &      gini &         5 &      200 &                             0.670683 &                                    0.684396 &                                     0.676057 &                          0.563005 \\
84 &         log2 &      gini &         6 &       50 &                             0.662545 &                                    0.671664 &                                     0.680674 &                          0.552235 \\
85 &         log2 &      gini &         6 &      100 &                             0.664043 &                                    0.679391 &                                     0.676820 &                          0.557692 \\
86 &         log2 &      gini &         6 &      150 &                             0.666477 &                                    0.674038 &                                     0.674768 &                          0.553892 \\
87 &         log2 &      gini &         6 &      200 &                             0.668189 &                                    0.678753 &                                     0.681144 &                          0.552462 \\
88 &         log2 &      gini &         8 &       50 &                             0.651327 &                                    0.666299 &                                     0.669061 &                          0.538158 \\
89 &         log2 &      gini &         8 &      100 &                             0.651179 &                                    0.667817 &                                     0.671680 &                          0.539468 \\
90 &         log2 &      gini &         8 &      150 &                             0.653840 &                                    0.669306 &                                     0.672931 &                          0.537264 \\
91 &         log2 &      gini &         8 &      200 &                             0.650357 &                                    0.661307 &                                     0.673223 &                          0.539444 \\
92 &         log2 &      gini &      None &       50 &                             0.583461 &                                    0.613313 &                                     0.659616 &                          0.538639 \\
93 &         log2 &      gini &      None &      100 &                             0.581805 &                                    0.615165 &                                     0.666460 &                          0.539151 \\
94 &         log2 &      gini &      None &      150 &                             0.580916 &                                    0.615916 &                                     0.663662 &                          0.542014 \\
95 &         log2 &      gini &      None &      200 &                             0.580624 &                                    0.621149 &                                     0.661692 &                          0.541741 \\
\bottomrule
\end{tabular}


==> tables_old/triton.3-_average_recall.tex <==
\begin{tabular}{llllrrrr}
\toprule
{} & max\_features & criterion & max\_depth &  n\_trees &  Scalar, all features average recall &  Scalar, restricted features average recall &  Encoded, restricted features average recall \\
\midrule
0  &         None &   entropy &        10 &       50 &                             0.863475 &                                    0.859715 &                                     0.843268 \\
1  &         None &   entropy &        10 &      100 &                             0.862993 &                                    0.860225 &                                     0.849932 \\
2  &         None &   entropy &        10 &      150 &                             0.862649 &                                    0.860167 &                                     0.848998 \\
3  &         None &   entropy &        10 &      200 &                             0.862321 &                                    0.856917 &                                     0.844391 \\
4  &         None &   entropy &         4 &       50 &                             0.856818 &                                    0.860418 &                                     0.845847 \\
5  &         None &   entropy &         4 &      100 &                             0.860009 &                                    0.862543 &                                     0.851835 \\
6  &         None &   entropy &         4 &      150 &                             0.860274 &                                    0.862513 &                                     0.847661 \\
7  &         None &   entropy &         4 &      200 &                             0.861247 &                                    0.860606 &                                     0.845425 \\
8  &         None &   entropy &         5 &       50 &                             0.852370 &                                    0.865764 &                                     0.861737 \\
9  &         None &   entropy &         5 &      100 &                             0.865085 &                                    0.867485 &                                     0.855898 \\
10 &         None &   entropy &         5 &      150 &                             0.862198 &                                    0.866510 &                                     0.858090 \\
11 &         None &   entropy &         5 &      200 &                             0.862073 &                                    0.864077 &                                     0.858828 \\
12 &         None &   entropy &         6 &       50 &                             0.869013 &                                    0.865441 &                                     0.861953 \\
13 &         None &   entropy &         6 &      100 &                             0.860248 &                                    0.866078 &                                     0.857004 \\
14 &         None &   entropy &         6 &      150 &                             0.860114 &                                    0.862933 &                                     0.858499 \\
15 &         None &   entropy &         6 &      200 &                             0.863454 &                                    0.865360 &                                     0.855738 \\
16 &         None &   entropy &         8 &       50 &                             0.863859 &                                    0.858933 &                                     0.854648 \\
17 &         None &   entropy &         8 &      100 &                             0.866289 &                                    0.860839 &                                     0.846697 \\
18 &         None &   entropy &         8 &      150 &                             0.866357 &                                    0.860864 &                                     0.853657 \\
19 &         None &   entropy &         8 &      200 &                             0.864813 &                                    0.863300 &                                     0.856822 \\
20 &         None &   entropy &      None &       50 &                             0.856291 &                                    0.851333 &                                     0.850282 \\
21 &         None &   entropy &      None &      100 &                             0.860492 &                                    0.861728 &                                     0.842287 \\
22 &         None &   entropy &      None &      150 &                             0.856296 &                                    0.862811 &                                     0.847888 \\
23 &         None &   entropy &      None &      200 &                             0.860766 &                                    0.853027 &                                     0.842058 \\
24 &         None &      gini &        10 &       50 &                             0.855378 &                                    0.852328 &                                     0.843527 \\
25 &         None &      gini &        10 &      100 &                             0.852816 &                                    0.851338 &                                     0.843401 \\
26 &         None &      gini &        10 &      150 &                             0.854743 &                                    0.854921 &                                     0.845077 \\
27 &         None &      gini &        10 &      200 &                             0.849846 &                                    0.853727 &                                     0.849522 \\
28 &         None &      gini &         4 &       50 &                             0.858279 &                                    0.861826 &                                     0.846254 \\
29 &         None &      gini &         4 &      100 &                             0.859819 &                                    0.862403 &                                     0.846842 \\
30 &         None &      gini &         4 &      150 &                             0.853517 &                                    0.866469 &                                     0.851147 \\
31 &         None &      gini &         4 &      200 &                             0.864079 &                                    0.861821 &                                     0.851464 \\
32 &         None &      gini &         5 &       50 &                             0.861182 &                                    0.861595 &                                     0.855004 \\
33 &         None &      gini &         5 &      100 &                             0.865467 &                                    0.856751 &                                     0.861191 \\
34 &         None &      gini &         5 &      150 &                             0.867107 &                                    0.864731 &                                     0.851815 \\
35 &         None &      gini &         5 &      200 &                             0.864971 &                                    0.861474 &                                     0.857429 \\
36 &         None &      gini &         6 &       50 &                             0.863364 &                                    0.862933 &                                     0.852024 \\
37 &         None &      gini &         6 &      100 &                             0.864930 &                                    0.859434 &                                     0.851065 \\
38 &         None &      gini &         6 &      150 &                             0.863085 &                                    0.858652 &                                     0.853342 \\
39 &         None &      gini &         6 &      200 &                             0.865225 &                                    0.856294 &                                     0.851089 \\
40 &         None &      gini &         8 &       50 &                             0.860238 &                                    0.858582 &                                     0.843344 \\
41 &         None &      gini &         8 &      100 &                             0.858735 &                                    0.857946 &                                     0.849695 \\
42 &         None &      gini &         8 &      150 &                             0.856088 &                                    0.855495 &                                     0.854662 \\
43 &         None &      gini &         8 &      200 &                             0.860497 &                                    0.854897 &                                     0.847729 \\
44 &         None &      gini &      None &       50 &                             0.853389 &                                    0.848398 &                                     0.839780 \\
45 &         None &      gini &      None &      100 &                             0.854870 &                                    0.853572 &                                     0.846954 \\
46 &         None &      gini &      None &      150 &                             0.849186 &                                    0.851895 &                                     0.843518 \\
47 &         None &      gini &      None &      200 &                             0.853050 &                                    0.854184 &                                     0.842082 \\
48 &         log2 &   entropy &        10 &       50 &                             0.865611 &                                    0.858582 &                                     0.857774 \\
49 &         log2 &   entropy &        10 &      100 &                             0.868077 &                                    0.856673 &                                     0.858045 \\
50 &         log2 &   entropy &        10 &      150 &                             0.866949 &                                    0.857399 &                                     0.854723 \\
51 &         log2 &   entropy &        10 &      200 &                             0.861799 &                                    0.860358 &                                     0.851516 \\
52 &         log2 &   entropy &         4 &       50 &                             0.864283 &                                    0.859728 &                                     0.850777 \\
53 &         log2 &   entropy &         4 &      100 &                             0.864386 &                                    0.863110 &                                     0.854163 \\
54 &         log2 &   entropy &         4 &      150 &                             0.862430 &                                    0.863754 &                                     0.851800 \\
55 &         log2 &   entropy &         4 &      200 &                             0.863577 &                                    0.861223 &                                     0.854834 \\
56 &         log2 &   entropy &         5 &       50 &                             0.867396 &                                    0.859608 &                                     0.858640 \\
57 &         log2 &   entropy &         5 &      100 &                             0.865995 &                                    0.860286 &                                     0.859181 \\
58 &         log2 &   entropy &         5 &      150 &                             0.869683 &                                    0.861088 &                                     0.858577 \\
59 &         log2 &   entropy &         5 &      200 &                             0.868484 &                                    0.865150 &                                     0.857605 \\
60 &         log2 &   entropy &         6 &       50 &                             0.866111 &                                    0.862805 &                                     0.858039 \\
61 &         log2 &   entropy &         6 &      100 &                             0.868097 &                                    0.865495 &                                     0.859177 \\
62 &         log2 &   entropy &         6 &      150 &                             0.865028 &                                    0.862841 &                                     0.856150 \\
63 &         log2 &   entropy &         6 &      200 &                             0.871413 &                                    0.864570 &                                     0.864547 \\
64 &         log2 &   entropy &         8 &       50 &                             0.862907 &                                    0.864368 &                                     0.855799 \\
65 &         log2 &   entropy &         8 &      100 &                             0.865080 &                                    0.864525 &                                     0.860495 \\
66 &         log2 &   entropy &         8 &      150 &                             0.862613 &                                    0.861096 &                                     0.865079 \\
67 &         log2 &   entropy &         8 &      200 &                             0.865004 &                                    0.860298 &                                     0.857770 \\
68 &         log2 &   entropy &      None &       50 &                             0.862614 &                                    0.854468 &                                     0.845424 \\
69 &         log2 &   entropy &      None &      100 &                             0.866716 &                                    0.855999 &                                     0.846361 \\
70 &         log2 &   entropy &      None &      150 &                             0.865708 &                                    0.856546 &                                     0.845845 \\
71 &         log2 &   entropy &      None &      200 &                             0.863853 &                                    0.855971 &                                     0.848437 \\
72 &         log2 &      gini &        10 &       50 &                             0.865754 &                                    0.860942 &                                     0.853000 \\
73 &         log2 &      gini &        10 &      100 &                             0.865517 &                                    0.855619 &                                     0.853761 \\
74 &         log2 &      gini &        10 &      150 &                             0.869306 &                                    0.856549 &                                     0.854258 \\
75 &         log2 &      gini &        10 &      200 &                             0.866433 &                                    0.860230 &                                     0.852866 \\
76 &         log2 &      gini &         4 &       50 &                             0.863465 &                                    0.859403 &                                     0.856628 \\
77 &         log2 &      gini &         4 &      100 &                             0.863480 &                                    0.862893 &                                     0.859254 \\
78 &         log2 &      gini &         4 &      150 &                             0.864853 &                                    0.859426 &                                     0.847884 \\
79 &         log2 &      gini &         4 &      200 &                             0.866162 &                                    0.864380 &                                     0.848208 \\
80 &         log2 &      gini &         5 &       50 &                             0.868532 &                                    0.859135 &                                     0.854218 \\
81 &         log2 &      gini &         5 &      100 &                             0.869192 &                                    0.866335 &                                     0.855697 \\
82 &         log2 &      gini &         5 &      150 &                             0.866840 &                                    0.858135 &                                     0.858691 \\
83 &         log2 &      gini &         5 &      200 &                             0.870039 &                                    0.861414 &                                     0.864270 \\
84 &         log2 &      gini &         6 &       50 &                             0.866636 &                                    0.862921 &                                     0.856239 \\
85 &         log2 &      gini &         6 &      100 &                             0.865743 &                                    0.862879 &                                     0.856694 \\
86 &         log2 &      gini &         6 &      150 &                             0.862546 &                                    0.864787 &                                     0.861586 \\
87 &         log2 &      gini &         6 &      200 &                             0.867911 &                                    0.860386 &                                     0.858923 \\
88 &         log2 &      gini &         8 &       50 &                             0.863021 &                                    0.858673 &                                     0.855897 \\
89 &         log2 &      gini &         8 &      100 &                             0.863869 &                                    0.861208 &                                     0.858509 \\
90 &         log2 &      gini &         8 &      150 &                             0.864180 &                                    0.860572 &                                     0.860500 \\
91 &         log2 &      gini &         8 &      200 &                             0.865559 &                                    0.861994 &                                     0.862692 \\
92 &         log2 &      gini &      None &       50 &                             0.865062 &                                    0.851424 &                                     0.844912 \\
93 &         log2 &      gini &      None &      100 &                             0.860445 &                                    0.853519 &                                     0.842001 \\
94 &         log2 &      gini &      None &      150 &                             0.855909 &                                    0.857287 &                                     0.850084 \\
95 &         log2 &      gini &      None &      200 &                             0.859118 &                                    0.859922 &                                     0.848739 \\
\bottomrule
\end{tabular}


==> tables_old/triton.4+_average_recall.tex <==
\begin{tabular}{llllrrrr}
\toprule
{} & max\_features & criterion & max\_depth &  n\_trees &  Scalar, all features average recall &  Scalar, restricted features average recall &  Encoded, restricted features average recall \\
\midrule
0  &         None &   entropy &        10 &       50 &                             0.809202 &                                    0.813124 &                                     0.826751 \\
1  &         None &   entropy &        10 &      100 &                             0.808237 &                                    0.805559 &                                     0.819527 \\
2  &         None &   entropy &        10 &      150 &                             0.810501 &                                    0.809402 &                                     0.824694 \\
3  &         None &   entropy &        10 &      200 &                             0.803447 &                                    0.808929 &                                     0.825720 \\
4  &         None &   entropy &         4 &       50 &                             0.868758 &                                    0.849287 &                                     0.890187 \\
5  &         None &   entropy &         4 &      100 &                             0.869930 &                                    0.851533 &                                     0.898182 \\
6  &         None &   entropy &         4 &      150 &                             0.869487 &                                    0.853676 &                                     0.894283 \\
7  &         None &   entropy &         4 &      200 &                             0.868740 &                                    0.851194 &                                     0.893393 \\
8  &         None &   entropy &         5 &       50 &                             0.854045 &                                    0.843200 &                                     0.879826 \\
9  &         None &   entropy &         5 &      100 &                             0.852333 &                                    0.843127 &                                     0.887426 \\
10 &         None &   entropy &         5 &      150 &                             0.856528 &                                    0.844712 &                                     0.883293 \\
11 &         None &   entropy &         5 &      200 &                             0.855241 &                                    0.844494 &                                     0.878661 \\
12 &         None &   entropy &         6 &       50 &                             0.841904 &                                    0.832942 &                                     0.867315 \\
13 &         None &   entropy &         6 &      100 &                             0.838621 &                                    0.823903 &                                     0.867412 \\
14 &         None &   entropy &         6 &      150 &                             0.834844 &                                    0.832396 &                                     0.865997 \\
15 &         None &   entropy &         6 &      200 &                             0.840169 &                                    0.828893 &                                     0.872098 \\
16 &         None &   entropy &         8 &       50 &                             0.814319 &                                    0.814877 &                                     0.832116 \\
17 &         None &   entropy &         8 &      100 &                             0.814532 &                                    0.815303 &                                     0.835054 \\
18 &         None &   entropy &         8 &      150 &                             0.809985 &                                    0.812303 &                                     0.834173 \\
19 &         None &   entropy &         8 &      200 &                             0.813367 &                                    0.808017 &                                     0.838168 \\
20 &         None &   entropy &      None &       50 &                             0.807945 &                                    0.810028 &                                     0.812638 \\
21 &         None &   entropy &      None &      100 &                             0.805894 &                                    0.805298 &                                     0.811520 \\
22 &         None &   entropy &      None &      150 &                             0.805924 &                                    0.803890 &                                     0.816128 \\
23 &         None &   entropy &      None &      200 &                             0.797904 &                                    0.803768 &                                     0.820263 \\
24 &         None &      gini &        10 &       50 &                             0.815461 &                                    0.800205 &                                     0.826811 \\
25 &         None &      gini &        10 &      100 &                             0.814988 &                                    0.808777 &                                     0.823484 \\
26 &         None &      gini &        10 &      150 &                             0.818891 &                                    0.803021 &                                     0.827788 \\
27 &         None &      gini &        10 &      200 &                             0.816396 &                                    0.804903 &                                     0.824632 \\
28 &         None &      gini &         4 &       50 &                             0.875332 &                                    0.856333 &                                     0.885010 \\
29 &         None &      gini &         4 &      100 &                             0.879509 &                                    0.854124 &                                     0.882983 \\
30 &         None &      gini &         4 &      150 &                             0.879357 &                                    0.854889 &                                     0.889742 \\
31 &         None &      gini &         4 &      200 &                             0.875459 &                                    0.851981 &                                     0.885582 \\
32 &         None &      gini &         5 &       50 &                             0.868723 &                                    0.846641 &                                     0.868869 \\
33 &         None &      gini &         5 &      100 &                             0.864480 &                                    0.843090 &                                     0.869896 \\
34 &         None &      gini &         5 &      150 &                             0.864201 &                                    0.845275 &                                     0.877650 \\
35 &         None &      gini &         5 &      200 &                             0.865652 &                                    0.845627 &                                     0.877103 \\
36 &         None &      gini &         6 &       50 &                             0.845401 &                                    0.834860 &                                     0.858748 \\
37 &         None &      gini &         6 &      100 &                             0.850591 &                                    0.834945 &                                     0.861590 \\
38 &         None &      gini &         6 &      150 &                             0.846178 &                                    0.833336 &                                     0.855585 \\
39 &         None &      gini &         6 &      200 &                             0.845553 &                                    0.828364 &                                     0.858305 \\
40 &         None &      gini &         8 &       50 &                             0.833594 &                                    0.811848 &                                     0.833784 \\
41 &         None &      gini &         8 &      100 &                             0.830425 &                                    0.813026 &                                     0.839211 \\
42 &         None &      gini &         8 &      150 &                             0.830316 &                                    0.812795 &                                     0.839654 \\
43 &         None &      gini &         8 &      200 &                             0.825587 &                                    0.812504 &                                     0.838592 \\
44 &         None &      gini &      None &       50 &                             0.802950 &                                    0.796647 &                                     0.812990 \\
45 &         None &      gini &      None &      100 &                             0.804419 &                                    0.802955 &                                     0.813858 \\
46 &         None &      gini &      None &      150 &                             0.807405 &                                    0.801025 &                                     0.807799 \\
47 &         None &      gini &      None &      200 &                             0.807327 &                                    0.799495 &                                     0.813433 \\
48 &         log2 &   entropy &        10 &       50 &                             0.805809 &                                    0.806701 &                                     0.812219 \\
49 &         log2 &   entropy &        10 &      100 &                             0.805748 &                                    0.804145 &                                     0.813701 \\
50 &         log2 &   entropy &        10 &      150 &                             0.805840 &                                    0.805311 &                                     0.814132 \\
51 &         log2 &   entropy &        10 &      200 &                             0.802258 &                                    0.799677 &                                     0.810975 \\
52 &         log2 &   entropy &         4 &       50 &                             0.898352 &                                    0.866240 &                                     0.868416 \\
53 &         log2 &   entropy &         4 &      100 &                             0.897430 &                                    0.872341 &                                     0.871304 \\
54 &         log2 &   entropy &         4 &      150 &                             0.900271 &                                    0.867783 &                                     0.872130 \\
55 &         log2 &   entropy &         4 &      200 &                             0.899245 &                                    0.867298 &                                     0.869555 \\
56 &         log2 &   entropy &         5 &       50 &                             0.883020 &                                    0.863979 &                                     0.878403 \\
57 &         log2 &   entropy &         5 &      100 &                             0.885928 &                                    0.863330 &                                     0.879376 \\
58 &         log2 &   entropy &         5 &      150 &                             0.883707 &                                    0.864320 &                                     0.881810 \\
59 &         log2 &   entropy &         5 &      200 &                             0.889893 &                                    0.862911 &                                     0.878452 \\
60 &         log2 &   entropy &         6 &       50 &                             0.853251 &                                    0.845836 &                                     0.871694 \\
61 &         log2 &   entropy &         6 &      100 &                             0.860184 &                                    0.850456 &                                     0.868294 \\
62 &         log2 &   entropy &         6 &      150 &                             0.865265 &                                    0.850086 &                                     0.871718 \\
63 &         log2 &   entropy &         6 &      200 &                             0.858132 &                                    0.848581 &                                     0.872939 \\
64 &         log2 &   entropy &         8 &       50 &                             0.819608 &                                    0.822557 &                                     0.837654 \\
65 &         log2 &   entropy &         8 &      100 &                             0.821733 &                                    0.817227 &                                     0.831881 \\
66 &         log2 &   entropy &         8 &      150 &                             0.819450 &                                    0.811411 &                                     0.836331 \\
67 &         log2 &   entropy &         8 &      200 &                             0.819760 &                                    0.814641 &                                     0.834619 \\
68 &         log2 &   entropy &      None &       50 &                             0.791464 &                                    0.800072 &                                     0.809943 \\
69 &         log2 &   entropy &      None &      100 &                             0.794220 &                                    0.801389 &                                     0.808535 \\
70 &         log2 &   entropy &      None &      150 &                             0.795246 &                                    0.795203 &                                     0.806301 \\
71 &         log2 &   entropy &      None &      200 &                             0.791142 &                                    0.797407 &                                     0.804862 \\
72 &         log2 &      gini &        10 &       50 &                             0.805427 &                                    0.804959 &                                     0.813336 \\
73 &         log2 &      gini &        10 &      100 &                             0.802762 &                                    0.802676 &                                     0.808650 \\
74 &         log2 &      gini &        10 &      150 &                             0.801553 &                                    0.802798 &                                     0.810945 \\
75 &         log2 &      gini &        10 &      200 &                             0.798445 &                                    0.802737 &                                     0.809827 \\
76 &         log2 &      gini &         4 &       50 &                             0.893276 &                                    0.869567 &                                     0.870868 \\
77 &         log2 &      gini &         4 &      100 &                             0.894631 &                                    0.868146 &                                     0.872961 \\
78 &         log2 &      gini &         4 &      150 &                             0.895451 &                                    0.868590 &                                     0.867326 \\
79 &         log2 &      gini &         4 &      200 &                             0.899367 &                                    0.870259 &                                     0.871570 \\
80 &         log2 &      gini &         5 &       50 &                             0.879244 &                                    0.862152 &                                     0.881197 \\
81 &         log2 &      gini &         5 &      100 &                             0.887251 &                                    0.864617 &                                     0.878932 \\
82 &         log2 &      gini &         5 &      150 &                             0.886505 &                                    0.864860 &                                     0.878035 \\
83 &         log2 &      gini &         5 &      200 &                             0.892674 &                                    0.866475 &                                     0.879728 \\
84 &         log2 &      gini &         6 &       50 &                             0.862132 &                                    0.848313 &                                     0.866503 \\
85 &         log2 &      gini &         6 &      100 &                             0.863614 &                                    0.854476 &                                     0.869867 \\
86 &         log2 &      gini &         6 &      150 &                             0.856936 &                                    0.850754 &                                     0.866492 \\
87 &         log2 &      gini &         6 &      200 &                             0.863596 &                                    0.849194 &                                     0.869818 \\
88 &         log2 &      gini &         8 &       50 &                             0.817908 &                                    0.819540 &                                     0.830916 \\
89 &         log2 &      gini &         8 &      100 &                             0.820294 &                                    0.813815 &                                     0.832919 \\
90 &         log2 &      gini &         8 &      150 &                             0.820829 &                                    0.817258 &                                     0.829441 \\
91 &         log2 &      gini &         8 &      200 &                             0.814952 &                                    0.813293 &                                     0.834923 \\
92 &         log2 &      gini &      None &       50 &                             0.791907 &                                    0.795646 &                                     0.804370 \\
93 &         log2 &      gini &      None &      100 &                             0.790438 &                                    0.795707 &                                     0.799902 \\
94 &         log2 &      gini &      None &      150 &                             0.794954 &                                    0.797085 &                                     0.798967 \\
95 &         log2 &      gini &      None &      200 &                             0.790025 &                                    0.796533 &                                     0.800989 \\
\bottomrule
\end{tabular}

